Evaluation of Transfer Learning for Classification of: (1) Diabetic Retinopathy by Digital Fundus Photography and (2) Diabetic Macular Edema, Choroidal Neovascularization and Drusen by Optical Coherence Tomography

Deep learning has been successfully applied to a variety of image classification tasks. There has been keen interest to apply deep learning in the medical domain, particularly specialties that heavily utilize imaging, such as ophthalmology. One issue that may hinder application of deep learning to the medical domain is the vast amount of data necessary to train deep neural networks (DNNs). Because of regulatory and privacy issues associated with medicine, and the generally proprietary nature of data in medical domains, obtaining large datasets to train DNNs is a challenge, particularly in the ophthalmology domain. Transfer learning is a technique developed to address the issue of applying DNNs for domains with limited data. Prior reports on transfer learning have examined custom networks to fully train or used a particular DNN for transfer learning. However, to the best of my knowledge, no work has systematically examined a suite of DNNs for transfer learning for classification of diabetic retinopathy, diabetic macular edema, and two key features of age-related macular degeneration. This work attempts to investigate transfer learning for classification of these ophthalmic conditions. Part I gives a condensed overview of neural networks and the DNNs under evaluation. Part II gives the reader the necessary background concerning diabetic retinopathy and prior work on classification using retinal fundus photographs. The methodology and results of transfer learning for diabetic retinopathy classification are presented, showing that transfer learning towards this domain is feasible, with promising accuracy. Part III gives an overview of diabetic macular edema, choroidal neovascularization and drusen (features associated with age-related macular degeneration), and presents results for transfer learning evaluation using optical coherence tomography to classify these entities.

==> OCT_results.tex <==
\chapter{Results\label{chap:OCT_results}}

There was a total of 64 runs (16 networks x pre-trained vs. not pre-trained x fine-tuning vs. fixed feature extractor). Detailed loss and accuracy plots for each run are plotted in appendix \ref{chap:append_network_plots}, specifically figures \ref{fig:AlexNet_acc_plt}-\ref{fig:Diabetic_Retinopathy_VGG-19_acc_plt}. The plots shows loss or accuracy data over 10 epochs, for training and validation. Each plot corresponds to one of the 64 network/pre-trained or not pre-trained/fine-tuning or fixed feature extractor combinations.\\
\indent Table \ref{tab:DR_loss_results} shows the loss results for the 16 networks that were evaluated. The results are grouped by not-pretrained and pre-trained catagories, then by training or validation phases, and lastly by the type of implementation (fine-tuning the network or using it as feature extractor). The results of this table are summarized in the series of boxplots in appendix \ref{chap:append_network_plots}, figure \ref{fig:DR_network_loss_boxplots}.

\begin{table}[htb!]
\caption[OCT: Network loss results]{\textbf{OCT: Network loss results.} Shown are the loss values for each network at the last epoch. Values are grouped by the phase (training or validation), and whether the network was used in fine-tuning or fixed feature extractor mode. All networks were trained for 10 epochs in fine-tuning mode and xxx epochs in fixed feature extractor mode.}\label{tab:OCT_loss_results}
  \begin{center}
\scalebox{0.7}{
  \begin{tabular}{|l|r|r|r|r|r|r|}
\toprule
& \multicolumn{2}{c}{\underline{\textbf{Training}}} & \multicolumn{2}{c}{\underline{\textbf{Validation}}} & &\\
& \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature} & \textbf{Fine Tuning} & \textbf{Feature Extractor}\\
\textbf{Network} & \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor} & \textbf{Training:Validation} & \textbf{Training:Validation}\\
& & & & & \textbf{Ratio} & \textbf{Ratio}\\
\midrule
AlexNet & 0.2557 & 0.7530 & 0.0498 & 0.5652 & 5.13 & 1.33\\
DenseNet-121 & & & & & &\\
DenseNet-169 & 0.1839 & 0.7346 & 0.0193 & 0.2018 & 9.52 & 3.64\\ 
DenseNet-201 & 0.1875 &  & 0.0197 & 9.52 & \\
Inception\_v3 & 0.1902 & 0.8710 & 0.0224 & 0.5022 & 8.49 & 1.73\\
ResNet-18 & 0.2086 & 0.7957 & 0.0289 & 0.3393 & 7.22 & 2.35\\
ResNet-34 & 0.1924 & 0.7802 & 0.0227 & 0.4159 & 8.47 & 1.86\\
ResNet-50 & 0.1933 & 0.6659 & 0.0315 & 0.3291 & 6.14 & 2.02\\
ResNet-101 & 0.1888 & 0.6737 & 0.0405 & 0.3760 & 4.66 & 1.79\\
ResNet-152 & 0.1825 & 0.6688 & 0.0212 & 2.4509 & 8.61 & 0.27\\
VGG-11 & 0.1978 & 0.7236 & 0.0205 & 0.4033 & 9.65 & 1.79\\
VGG-11bn & 0.1909 & 0.8011 & 0.0118 & 0.5672 & 16.18 & 1.41\\
VGG-13 & 0.1976 & 0.6863 & 0.0502 & 0.3753 & 3.94 & 1.83\\
VGG-16 & 0.1929 & 0.7104 & 0.0170 & 0.4279 & 11.35 & 1.66\\
VGG-19 & 0.1927 & 0.7134 & 0.0154 & 0.3417 & 12.51 & 2.09\\
\bottomrule
\end{tabular}}
\end{center}
\end{table}

\indent Similarly, table \ref{tab:OCT_acc_results} shows the accuracy results for the networks that were evaluated. The results in that table are also grouped by training or validation phases, and by the type of implementation (fine-tuning the network or using it as feature extractor). The results of this table are summarized in the series of boxplots in appendix \ref{chap:append_network_plots}, figure \ref{fig:DR_network_acc_boxplots}.

\begin{table}[htb!]
\caption[OCT: Network accuracy results]{\textbf{OCT: Network accuracy results.} Shown are the accuracy values for each network at the last epoch for training phase and the best accuracy for validation phase. Values are grouped by phase (training or validation), and whether the network was used in fine-tuning or fixed feature extractor mode. All networks were trained for 10 epochs in fine-tuning and xxx epochs in fixed feature extractor.}\label{tab:OCT_acc_results}
  \begin{center}
\scalebox{0.7}{
  \begin{tabular}{|l|r|r|r|r|}
\toprule
& \multicolumn{2}{c}{\underline{\textbf{Training Accuracy}}} & \multicolumn{2}{c}{\underline{\textbf{Validation Accuracy}}}\\
& \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature}\\
\textbf{Network} & \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor}\\
\midrule
AlexNet & 0.9068 & 0.7235  & 1.0000 & 0.8125\\
DenseNet-121 & & & &\\
DenseNet-169 & 0.9326 & 0.7196 & 1.0000 & 0.9375\\
DenseNet-201 & 0.9304 &        & 1.0000 & \\
Inception\_v3 & 0.9304 & 0.6610 & 1.0000 & 0.9063\\
ResNet-18 & 0.9235 & 0.6922 & 1.0000 & 0.9063\\
ResNet-34 & 0.9294 & 0.7009 & 1.0000 & 0.9063\\
ResNet-50 & 0.9294 & 0.7479 & 1.0000 & 0.9063\\
ResNet-101 & 0.9299 & 0.7458 & 1.0000 & 0.9063\\
ResNet-152 & 0.9322 & 0.7464 & 1.0000 & 0.9375\\
VGG-11 & 0.9269 & 0.7291& 1.0000 & 0.8750\\
VGG-11bn & 0.9290 & 0.6938 & 1.0000 & 0.8125\\
VGG-13 & 0.9281 & 0.7446 & 1.0000 & 0.9375\\ 
VGG-16 & 0.9286 & 0.7334 & 1.0000 & 0.9063\\
VGG-19 & 0.9303 & 0.7313 & 1.0000 & 0.9375\\

\bottomrule 
\end{tabular}}
\end{center}
\end{table}

%Table \ref{tab:DR_loss_stats} summarizes the mean, standard deviation, and median values for loss across the models for the various combinations pre-trained vs. not pretrained, training vs. validation phases, and fine-tuning vs. feature-extractor. Table \ref{tab:DR_acc_stats} similarly does so for the accuracy.
%
%\begin{table}[htb!]
%\caption[Diabetic retinopathy: Network loss statistics]{\textbf{Diabetic retinopathy: Network loss statistics.} Shown are the mean, standard deviation, and median values for the loss data at the last epoch. Results are across the 16 networks evaluated and are grouped by pre-trained vs. not pre-trained networks, training or validation phase, and whether the networks were used as fine-tuning or as fixed feature extractors.}\label{tab:DR_loss_stats}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{l|r|r|r|r|r|r|r|r}
%\toprule
%& \multicolumn{4}{c}{\underline{\textbf{Not-Pretrained}}} & \multicolumn{4}{c}{\underline{\textbf{Pre-Trained}}}\\
%& \multicolumn{2}{c}{\underline{\textbf{Training}}} & \multicolumn{2}{c}{\underline{\textbf{Validation}}} & \multicolumn{2}{c}{\underline{\textbf{Training}}} & \multicolumn{2}{c}{\underline{\textbf{Validation}}}\\
%& \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature}\\
%& \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor}\\
%\midrule
%Mean & 0.846 & 0.979 & 0.972 & 0.901 & 0.649 & 0.885 & 0.718 & 0.901\\
%Stdv & 0.059 & 0.336 & 0.195 & 0.048 & 0.063 & 0.112 & 0.242 & 0.325\\
%Median & 0.861 & 0.876 & 0.880 & 0.889 & 0.626 & 0.822 & 0.644 & 0.814\\
%\bottomrule
%\end{tabular}}
%\end{center}
%\end{table}
%
%\begin{table}[htb!]
%\caption[Diabetic retinopathy: Network accuracy statistics]{\textbf{Diabetic retinopathy: Network accuracy stastistics}. Shown are the mean, standard deviation, and median values for the accuracy data (best accuracy over the epochs). Results are across the 16 networks evaluated and are grouped by pre-trained vs. not pre-trained networks, training or validation phase, and whether the networks were used as fine-tuning or as fixed feature extractors.}\label{tab:DR_acc_stats}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{l|r|r|r|r|r|r|r|r}
%\toprule
%& \multicolumn{4}{c}{\underline{\textbf{Not-Pretrained}}} & \multicolumn{4}{c}{\underline{\textbf{Pre-Trained}}}\\
%& \multicolumn{2}{c}{\underline{\textbf{Training}}} & \multicolumn{2}{c}{\underline{\textbf{Validation}}} & \multicolumn{2}{c}{\underline{\textbf{Training}}} & \multicolumn{2}{c}{\underline{\textbf{Validation}}}\\
%& \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature}\\
%& \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor}\\
%\midrule
%Mean & 0.739 & 0.721 & 0.739 & 0.735 & 0.786 & 0.720 & 0.790 & 0.740\\
%Stdv & 0.015 & 0.033 & 0.015 & 0.001 & 0.018 & 0.026 & 0.019 & 0.005\\
%Median & 0.735 & 0.735 & 0.735 & 0.735 & 0.792 & 0.734 & 0.796 & 0.741\\
%\bottomrule
%\end{tabular}}
%\end{center}
%\end{table}
%
%\indent From tables \ref{tab:DR_loss_results}-\ref{tab:DR_acc_stats} and the boxplots \ref{fig:DR_network_loss_boxplots} and \ref{fig:DR_network_acc_boxplots} in appendix \ref{chap:append_network_plots}, several observations are made:\\
%\\
%(1) The loss was generally lower in the pre-trained models compared to the not pre-trained models when comparing fixed pairs of fine-tuning or feature extractor and training or validation phases. For instance, the losses in the pre-trained validation phase for fine-tuning were lower than that of not pre-trained validation phase for fine-tuning. These trends were graphically observed in the boxplots in appendix \ref{chap:append_network_plots}, in particular figure \ref{fig:DR_loss_boxplots_a}-\ref{fig:DR_loss_boxplots_d}, shows that the pre-trained group has lower loss than the not pre-trained group. This was confirmed in table \ref{tab:DR_loss_acc_comparisons}, which showed that there were statistically significant differences for each of the pairwise pre-trained vs. not pre-trained comparisons, except for the pretrained vs. not-pretrained training phase feature-extractor comparison (corresponds to figure \ref{fig:DR_loss_boxplots_b} (see table \ref{tab:DR_loss_acc_comparisons} test no. 2). The accuracy results showed the inverse pattern as the loss results, whereby the accuracy was higher in 3 of 4 cases for pre-trained networks (see table \ref{tab:DR_acc_results}, table \ref{tab:DR_acc_stats}, table \ref{tab:DR_loss_acc_comparisons} [test no. 1-4], and the boxplots in figure \ref{fig:DR_acc_boxplots_a}-\ref{fig:DR_acc_boxplots_d}).\\
%\begin{table}[htb!]
%\caption[Diabetic retinopathy: Network loss and accuracy comparisons]{\textbf{Diabetic retinopathy: Network loss and accuracy comparisons}. Shown are pair-wise Wilcoxon signed-rank (Test no. 1-8) or Mann-Whitney (Test no. 9-12) comparison tests between two catagories, where 2 of 3 variables (pre-trained vs. not pretrained, training or validation phase, fine-tuning vs. fixed feature extractor) were held fixed and the other varied. p-values are indicated, where p $<$ 0.05 (marked in bold) indicates a statistically significant difference between the two categories.}\label{tab:DR_loss_acc_comparisons}
%  \begin{center}
%\scalebox{0.6}{
%  \begin{tabular}{l|l|l|r|r}
%\toprule
%& \multicolumn{2}{c}{\textbf{Category}} & \multicolumn{2}{c}{\textbf{p-value}}\\
%\textbf{Test no.} & \textbf{A} & \textbf{B} & \textbf{Loss} & \textbf{Accuracy}\\
%\midrule
%1 & Not pretrained network/training phase/fine-tuning & Pretrained network/training phase/fine-tuning & \textbf{0.002} & \textbf{0.004}\\
%2 & Not pretrained network/training phase/feature-extractor & Pretrained network/training phase/feature extractor & 0.301 & 0.642\\
%3 & Not pretrained network/validation phase/fine-tuning & Pretrained network/validation phase/fine-tuning & \textbf{0.002} & \textbf{0.003}\\
%4 & Not pretrained network/validation phase/feature-extractor & Pretrained network/validation phase/feature extractor & \textbf{0.034} & \textbf{0.006}\\
%& & & \\
%5 & Not pretrained network/training phase/feature extractor & Not pretrained network/training phase/fine-tuning & \textbf{$<$0.001} & \textbf{0.005}\\
%6 & Not pretrained network/validation phase/feature extractor & Not pretrained network/validation phase/fine-tuning & 0.569 & 0.248\\
%7 & Pretrained network/training phase/feature extractor & Pretrained network/training phase/fine-tuning & \textbf{$<$0.001} & \textbf{0.001}\\
%8 & Pretrained network/validation phase/feature extractor & Pretrained network/validation phase/fine-tuning & \textbf{0.006} & \textbf{0.001}\\
%& & &\\
%9 & Not pretrained/training phase/fine-tuning & Not pretrained/validation phase/fine-tuning & 0.053 & \textbf{0.003}\\
%10 & Not pretrained network/training phase/feature extractor & Not pretrained network/validation phase/feature extractor & 0.462 & \textbf{$<$0.001}\\
%11 & Pretrained network/training phase/fine-tuning & Pretrained network/vaidation phase/fune-tuning & 0.220 & 0.146\\
%12 & Pretrained network/training phase/feature extractor & Pretrained network/validation phase/feature extractor & 0.084 & \textbf{$<$0.001}\\
%\bottomrule
%\end{tabular}}
%\end{center}
%\end{table}
%
%(2) Holding the pre-trained or not pre-trained variable fixed, the loss for fine-tuning was generally lower than that for feature-extractor, in both the training and validation phases (see boxplots \ref{fig:DR_loss_boxplots_e}-\ref{fig:DR_loss_boxplots_h}). These differenes were statistically significant except for the not pre-trained fine-tuning vs. feature extractor comparison in the validation phase (see figure \ref{fig:DR_loss_boxplots_f} and table \ref{tab:DR_loss_acc_comparisons} test no. 6). The accuracy results showed the inverse pattern as the loss results, whereby the accuracy was higher in 3 of 4 cases for fine-tuning (see table \ref{tab:DR_acc_results}, table \ref{tab:DR_acc_stats}, table \ref{tab:DR_loss_acc_comparisons} [test no. 5-8], and the boxplots in figure \ref{fig:DR_acc_boxplots_e}-\ref{fig:DR_acc_boxplots_h}).\\
%\\
%(3) The last group of comparisons held the pre-training vs. not pre-training variable fixed and the fine-tuning vs. feature extractor variable fixed, while evaluating for a difference between the training and validation phases. As indicated in table \ref{tab:DR_loss_acc_comparisons} there were no statistically differences for pair-wise comparisons between training and validation losses while holding the pre-trained/not pre-trained and fine-tuning/feature extractor variables fixed. Moreover, the values in tables \ref{tab:DR_acc_results}[test no. 9-12] and \ref{tab:DR_acc_stats}, and the boxplots in figure \ref{fig:DR_loss_boxplots_i}-\ref{fig:DR_loss_boxplots_l} indicate that the losses are very similar between the pairs. Table \ref{tab:DR_loss_acc_comparisons} indicates that there was a stastically significance between the training and validation groups for 3 of the 4 cases, with the exception (see table \ref{tab:DR_loss_acc_comparisons} test no. 11) being when the models were pre-trained and used as fine-tuning (see figure \ref{fig:DR_acc_boxplots_i}-\ref{fig:DR_acc_boxplots_l}).\\
%\\
%(4) Batch normalization(BN), applied to VGG-11, had mixed results. In the not pre-trained cases, the loss increased and the accuracy decreased compared to VGG withouth BN. In the pre-trained cases, the loss decreased and the accuracy increased in 3 of 4 cases (the exception being training accuracy as fixed feature extractor). In the pretrained, fine-tuning case validation accuracy substantially increased by 6.53\%, and was comparable in accuracy to VGG-19 without BN.
%
%
%\indent To evaluate for under- or over-fitting of the networks, the training to validation loss ratios were tabulated (table \ref{tab:DR_ratio_stats}) and plotted (figure \ref{fig:DR_ratio_boxplots}). The following patterns are observed:
%\begin{itemize}
%\item AlexNet had a ratio near 1, across the type of training and fine-tuning vs. fixed feature extractor mode.
%\item The DenseNet variants had ratios $<$1 when not pretrained, indicating these networks have higher validation loss than training loss and may be overfitting. However, when pretrained their ratios increased to $>$1, implying that overfitting is not likely present.
%item Inception\_v3 showed a similar pattern when not pretrained and pretrained: the fine-tuning ratios were $<$1, implying over-fitting, while the fixed feature extractor ratios were $>$1.
%\item The ResNet variants showed differing ratios: not pre-trained fine-tuning ratios were all $<$1, while pretrained fine-tuning were $>$1, execept for ResNet-101 and ResNet-152. The ResNet variants showed mixed ratios (table \ref{tab:DR_ratio_stats} as fixed feature extractors. ResNet-101 suffered a high validation loss when pre-trained as a fixed feature extractor, leading to an outlier ratio of 0.274.
%\item The VGG variants had ratios $>$1 across the combinations of pretrained or not pretrained and fine-tuning or fixed feature extractor, implying these networks were not over-fitting.
%\item When networks were not-pretrained and in fine-tuning mode, 10/16 (62.5\%) had ratios $<$1.
%\item When networks were not-pretrained and in fixed feature extractor mode, 6/16 (37.5\%) had ratios $<$1.
%\item When networks were pretrained and in fine-tuning mode, 3/16 (18.75\%) had ratios $<$1.
%\item When networks were pretrained and in fixed feature extrator mode, 4/16 (25\%) had ratios $<$1.
%\end{itemize}
%
%\begin{figure}[htb]
%%\begin{center}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{boxplot_not_pretrained_feature.png}
%\caption{Not pre-trained, fixed feature extractor.}
%\label{fig:DR_ratio_boxplots_a}
%\end{subfigure}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{boxplot_not_pretrained_fine_tune.png}
%\caption{Not pre-trained, fine-tuning.}
%\label{fig:DR_ratio_boxplots_b}
%\end{subfigure}
%\label{fig:DR_ratio_boxplots}
%\caption[Diabetic Retinopathy: Network training to validation ratio boxplots.]{\textbf{Diabetic Retinopathy: Network training to validation ratio boxplots.} Plotted are the training to validation ratios for each network. A ratio $<$1 implies over-fitting of the network.}\label{fig:DR_ratio_boxplots}
%\end{figure}
%
%\begin{figure}
%\ContinuedFloat
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{boxplot_pretrained_feature.png}
%\caption{Pre-trained, fixed feature extractor.}
%\label{fig:DR_ratio_boxplots_c}
%\end{subfigure}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{boxplot_not_pretrained_fine_tune.png}
%\caption{Pre-trained, fine-tuning.}
%\label{fig:DR_ratio_boxplots_d}
%\end{subfigure}
%\caption[Continued - Diabetic Retinopathy: Network training to validation ratio boxplots.]{\textbf{Continued - Diabetic Retinopathy to Network training to validation ratio boxplots.} A ratio $<$1 implies over-fitting of the network.}
%\label{fig:DR_ratio_boxplots2}
%\end{figure}
%
%
%\begin{table}[htb!]
%\caption[Diabetic retinopathy: Network training to validation ratio statistics]{\textbf{Diabetic retinopathy: Network training to validation ratio statistics.} Shown are the training to validation ratios for each network, grouped by pre-trained vs. not-pretrained network, training vs. validation phase, and whether the network was used in fine-tuning or fixed feature extrator mode.}\label{tab:DR_ratio_stats}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{|l|r|r|r|r|}
%\toprule
%& \multicolumn{2}{c}{\underline{\textbf{Not-Pretrained}}} & \multicolumn{2}{c}{\underline{\textbf{Pre-Trained}}}\\ 
%\textbf{Network} & \textbf{Fine} & \textbf{Feature} & \textbf{Fine} & \textbf{Feature}\\
%& \textbf{Tuning} & \textbf{Extractor} & \textbf{Tuning} & \textbf{Extractor}\\
%\midrule
%AlexNet & 1.004(0.005) & 1.004(0.007) & 1.019(0.011) & 1.168(0.093)\\
%DenseNet-121 & 0.823(0.156) & 0.938(0.058) & 1.019(1.019) & 1.009(0.095)\\
%DenseNet-161 & 0.789(0.150) & 0.845(0.101) & 1.024(0.060) & 1.013(0.080)\\
%DenseNet-169 & 0.802(0.180) & 0.802(0.180) & 1.015(0.065) & 1.055(0.083)\\
%DenseNet-201 & 0.691(0.261) & 0.857(0.125) & 1.017(0.059) & 1.066(0.050)\\
%Inception-v3 & 0.922(0.102) & 1.032(0.138) & 0.962(0.055) & 1.130(0.054)\\
%ResNet-18 & 0.998(0.010) & 0.974(0.082) & 1.016(0.047) & 0.988(0.088)\\
%ResNet-34 & 0.976(0.043) & 0.974(0.082) & 1.005(0.062) & 1.034(0.079)\\
%ResNet-50 & 0.743(0.260) & 1.244(0.301) & 1.016(0.044) & 0.947(0.134)\\
%ResNet-101 & 0.759(0.123) & 1.119(0.255) & 0.912(0.174) & 0.274(0.119)\\
%ResNet-152 & 0.701(0.117) & 1.096(0.253) & 0.836(0.216) & 0.943(0.122)\\
%VGG-11 & 1.006(0.005) & 1.011(0.005) & 1.025(0.032) & 1.341(0.159)\\
%VGG-11bn & 1.010(0.027) & 2.220(0.483) & 1.031(0.023) & 1.305(0.137)\\
%VGG-13 & 1.005(0.005) & 1.010(0.007) & 1.058(0.023) & 1.223(0.190)\\
%VGG-16 & 1.005(0.005) & 1.010(0.003) & 1.032(0.032) & 1.252(0.218)\\
%VGG-19 & 1.005(0.005) & 1.011(0.003) & 1.026(0.030) & 1.230(0.156)\\
%\bottomrule
%\end{tabular}}
%\end{center}
%\end{table}
%
%\indent Five of the 16 networks were selected for further evaluation with the test dataset. AlexNet and Inception\_v3 were selected along with one each of the ``best'' variants of ResNet, DenseNet, and VGG. ResNet-18 was selected because it had comparable accuracy (while minimizing complexity) to the other ResNet variants (table \ref{tab:DR_acc_results}) and a ratio near 1 when pretrained in fine-tuning mode. DenseNet-161 had highest accuracy when pretrained and in fine-tuning mode (table \ref{tab:DR_acc_results}) and had a ratio $>$1 with these parameters. Lastly, VGG-19 was near the top in validation accuracy when pretrained and in fine-tuning mode (table \ref{tab:DR_acc_results}) and had a ratio $>$1.\\
%\indent Accuracy of these 5 networks (pretrained) as fixed feature extractors or in fine-tuning mode when run with the test dataset is shown in table \ref{tab:DR_test_accuracy}. With fixed feature extractor, 4 of 5 networks had accuracy around 72-73\%, while DenseNet-161 had lower accuracy around 68\%. With fine-tuning, AlexNet and Inception\_v3 had about 3-4\% lower accuracy than the other 3 networks. DenseNet-161, ResNet-18, and VGG-19 had comparable accuracy around 76-77\%.\\
%
%\begin{table}[htb!]
%\caption[Diabetic retinopathy: Network Test Accuracy]{\textbf{Diabetic retinopathy: Network Test Accuracy}. Accuracy(\%) is indicated for the specified networks (all pre-trained) for fixed feature extractor and fine tuning modes.}\label{tab:DR_test_accuracy}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{|l|r|r|}
%\hline
%\textbf{Network} & \textbf{Fixed Feature Extractor} & \textbf{Fine-Tuning}\\
%\hline
%AlexNet & 72.2 & 73.6\\
%DenseNet-161 & 68.3 & 77.5\\
%Inception-v3 & 73.7 & 73.8\\
%ResNet-18 & 72.8 & 76.1\\
%VGG-19 & 73.2 & 77.4\\
%\hline
%\end{tabular}}
%\end{center}
%\end{table}
%
%\indent Quadratic weighted kappa was tabulated for each of the 5 networks (table \ref{tab:DR_test_kappa}). In fixed feature extractor mode, Inception\_v3 and VGG-19 showed poor level of agreement, while AlexNet, DenseNet-161, and ResNet-18 showed fair agreement. In fine-tuning mode, AlexNet and Inception\_v3 showed poor level of agreement, while DenseNet-161, ResNet-18, and VGG-19 showed moderate level of agreement.
%
%\begin{table}[htb!]
%\caption[Diabetic retinopathy: Network Test Quadratic Weighted Kappa]{\textbf{Diabetic retinopathy: Network Test Quadratic Weighted Kappa.} Quadratic weighted kappa values are indicated for the specified networks (all pre-trained) for fixed feature extractor and fine tuning modes. A generally agreed upon scale is: $<$0.20(Poor), 0.21-0.40(Fair), 0.41-0.60(Moderate), 0.61-0.80(Good), and 0.81-1.00(Very good).}\label{tab:DR_test_kappa}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{|l|r|r|}
%\hline
%\textbf{Network} & \textbf{Fixed Feature Extractor} & \textbf{Fine-Tuning}\\
%\hline
%AlexNet & 0.21 & 0.18\\
%DenseNet-161 & 0.32 & 0.55\\
%Inception-v3 & 0.005 & 0.15\\
%ResNet-18 & 0.23 & 0.47\\
%VGG-19 & 0.16 & 0.56\\
%\hline
%\end{tabular}}
%\end{center}
%\end{table}
%
%\indent Sensitivity and specificity were tabulated for each of the 5 networks (table \ref{tab:DR_s_and_s}). Since sensitivity and specificity are based on a binary classification, they were calculated in two ways: (1) for ``any DR,'' whereby the binary classification was normal (Class 0) vs. any level of DR (Class 1, 2, 3, or 4); and (2) ``referable DR,'' whereby the binary classification was non-referable (Class 0 or 1) vs. referable (Class 2, 3, or 4). Table \ref{tab:DR_s_and_s} shows that:
%\begin{itemize}
%\item Sensitivity was generally low for all the networks whether fine-tuning vs. fixed feature extractor.
%\item Sensitivity was in all cases higher for fine-tuning compared to fixed feature extractor. For VGG-19, it was substantially higher (57.2\% vs. 8.3\%).
%\item The highest sensitivity was achieved by VGG-19 (fine-tuning).
%\item Inception\_v3 showed poor sensitivity.
%\item Specificity was generally high ($>$94\%) for all the networks (fine-tuning).
%\end{itemize}
%
%\begin{table}[htb!]
%\caption[Diabetic retinopathy: Network Test Sensitivity and Specificity]{\textbf{Diabetic retinopathy: Network Test Sensitivity and Specificity.} Sensitivity(\%) and specificityi(\%) values are indicated for the specified networks (all pre-trained) for fixed feature extractor and fine tuning modes. Any DR indicates any level of diabetic retinopathy, referable DR indicates referable diabetic retinopathy, which is class 2 or higher (i.e., moderate diabetic retinopathy or worse).}\label{tab:DR_s_and_s}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{|l|r|r|r|r|r|r|r|r|r}
%\toprule
%& \multicolumn{4}{c}{\textbf{\underline{Fixed Feature Extractor}}} & \multicolumn{4}{c}{\textbf{\underline{Fine-tuning}}}\\
%& \multicolumn{2}{c}{\textbf{\underline{Any DR}}} & \multicolumn{2}{c}{\textbf{\underline{Referable DR}}} & \multicolumn{2}{c}{\textbf{\underline{Any DR}}} & \multicolumn{2}{c}{\textbf{\underline{Referable DR}}}\\
%\textbf{Network} & \textbf{Sensitivity} & \textbf{Specificity} & \textbf{Sensitivity} & \textbf{Specificity} & \textbf{Sensitivity} & \textbf{Specificity} & \textbf{Sensitivity} & \textbf{Specificity}\\
%\midrule
%AlexNet & 10.8 & 96.6 & 13.7 & 96.7 & 12.1 & 97.3 & 15.7 & 97.3\\
%DenseNet-161 & 34.6 & 85.5 & 41.2 & 85.3 & 41.6 & 95.1 & 54.1 & 94.9\\
%Inception-v3 & 3.0 & 99.9 & 4.0 & 99.9 & 10.5  & 97.6 & 13.3 & 97.8\\
%ResNet-18 & 13.7 & 96.1 & 17.3 & 96.2 & 33.9 & 95.4 & 44.3 & 95.3\\
%VGG-19 & 6.7 & 98.2 & 8.3 & 98.4 & 44.9 & 94.4 & 57.2 & 94.1\\
%\bottomrule
%\end{tabular}}
%\end{center}
%\end{table}
%
%\indent A selected subset of networks (DenseNet-161, Inception\_v3, ResNet-18, and VGG-19) were rerun (as pretrained, fine-tuning) for 50 epochs. Their loss and accuracy curves are plotted in figure \ref{fig:DR_50_epochs}. These plots show that the loss and accuracy begin to converge at around 10 epochs for these networks and there is minimal improvement in loss or accuracy past 10 epochs.
%
%\begin{figure}[htb]
%%\begin{center}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_resnet18_fine_tune_50_loss_epochs.png}
%\caption{Loss for ResNet-18.}
%\label{fig:DR_50_epochs_a}
%\end{subfigure}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_resnet18_fine_tune_50_acc_epochs.png}
%\caption{Accuracy for ResNet-18.}
%\label{fig:DR_50_epochs_b}
%\end{subfigure}
%\caption[Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.]{\textbf{Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.} Mode was set to fine-tuning.}\label{fig:DR_50_epochs}
%\end{figure}
%
%\begin{figure}
%\ContinuedFloat
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_inception_fine_tune_50_loss_epochs.png}
%\caption{Loss for Inception\_v3.}
%\label{fig:DR_50_epochs_c}
%\end{subfigure}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_inception_fine_tune_50_acc_epochs.png}
%\caption{Accuracy for Inception\_v3.}
%\label{fig:DR_50_epochs_d}
%\end{subfigure}
%\caption[Continued - Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.]{\textbf{Continued - Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.} Mode was set to fine-tuning}\label{fig:DR_50_epochs2}
%\end{figure}
%
%
%\begin{figure}
%\ContinuedFloat
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_densenet161_fine_tune_50_loss_epochs.png}
%\caption{Loss for Densenet-161.}
%\label{fig:DR_50_epochs_c}
%\end{subfigure}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_densenet161_fine_tune_50_acc_epochs.png}
%\caption{Accuracy for Densenet-161.}
%\label{fig:DR_50_epochs_d}
%\end{subfigure}
%\caption[Continued - Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.]{\textbf{Continued - Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.} Mode was set to fine-tuning}\label{fig:DR_50_epochs3}
%\end{figure}
%
%\begin{figure}
%\ContinuedFloat
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_vgg19_fine_tune_50_loss_epochs.png}
%\caption{Loss for VGG-19.}
%\label{fig:DR_50_epochs_c}
%\end{subfigure}
%\begin{subfigure}{0.8\textwidth}
%\captionsetup{width=0.8\textwidth}
%%\captionsetup[subfigure]{labelformat=empty}
%\centering\includegraphics[width=0.8\linewidth]{pretrained_vgg19_fine_tune_50_acc_epochs.png}
%\caption{Accuracy for VGG-19.}
%\label{fig:DR_50_epochs_d}
%\end{subfigure}
%\caption[Continued - Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.]{\textbf{Continued - Diabetic Retinopathy: Selected networks loss and accuracy curves over 50 epochs.} Mode was set to fine-tuning}\label{fig:DR_50_epochs4}
%\end{figure}
%
%\indent The effect of image pre-processing (see pre-processing methodology in chapter \ref{chap:DR_methods}) was analyzed for selected networks (AlexNet, DenseNet-161, Inception\_v3, ResNet-18, and VGG-19). Networks were pre-trained and used for fine-tuning and run for 10 epochs. Table \ref{tab:DR_image_preprocessing} shows there was minimal improvement of loss and accuracy for AlexNet, DenseNet-161 or ResNet-18. The validation accuracy for VGG-19 decreased very slightly (0.66\%). For Inception\_v3, there was a significant improvement in validation accuracy (6\%). 
%
%\begin{table}[htb!]
%\caption[Diabetic Retinopathy: Loss and Accuracy with image pre-processing.]{\textbf{Diabetic Retinopathy: Loss and Accuracy with image pre-processing.} Shown are the loss and accuracy for selected networks, comparing these values between runs with and without image pre-processng. Networks were pre-trained, run in fine-tuning mode for 10 epochs.}\label{tab:DR_image_preprocessing}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{|l|r|r|r|r|}
%\toprule
%& \multicolumn{2}{c}{\textbf{\underline{Loss}}} & \multicolumn{2}{c}{\textbf{\underline{Accuracy}}}\\
%\textbf{Network} & \textbf{Training} & \textbf{Validation} & \textbf{Training} & \textbf{Validation}\\
%\midrule
%AlexNet, without pre-processing & 0.7475 & 0.7431 & 0.7520 & 0.7579\\
%AlexNet, with pre-processing & 0.7475 & 0.7402 & 0.7524 & 0.7528\\
%DenseNet-161, without pre-processing & 0.6067 & 0.6162 & 0.8003 & 0.8038 \\
%DenseNet-161, with pre-processing & 0.5808 & 0.5946 & 0.8073 & 0.8105\\
%Inception\_v3, without pre-processing & 0.6368 & 0.6923 & 0.7896 & 0.7368 \\
%Inception\_v3, with pre-processing, & 0.5996 & 0.6401 & 0.8013 & 0.7974\\
%ResNet-18, without pre-processing & 0.6467 & 0.6616 & 0.7847 & 0.7952\\
%ResNet-18, with pre-processing & 0.6271 & 0.6177 & 0.7927 & 0.7969\\
%VGG-19, without pre-processing & 0.6055 & 0.5985 & 0.7990 & 0.8106\\
%VGG-19, with pre-processing & 0.5975 & 0.5995 & 0.8018 & 0.8040\\
%\bottomrule
%\end{tabular}}
%\end{center}
%\end{table}
%
%\indent The effect of adjusting class weights to account for class imbalance was investigated. VGG-19 (pretrained, fine-tuning) was re-run using various class-adjusted weights specified in table \ref{tab:DR_class_weighted}. The weights were adjusted to weigh class 0 (normal) less than the other classes. One recommendation was to use weights corresponding to the inverse of the class size, which is the second row in table {\ref{tab:DR_class_weighted}. Other class weights were experimented. The results indicated that adjusting the weights did not lower the loss or increase the accuracy over equally weighted classes.
%
%\begin{table}[htb!]
%\caption[Diabetic Retinopathy: VGG-19 class-weighted loss and accuracy.]{\textbf{Diabetic Retinopathy: VGG-19 class-weighted loss and accuracy.} Shown are the class-weighted loss and accuracy for VGG-19, run as pre-trained in fine-tuning mode for 10 epochs. For comparison reference, the first row is the result from table \ref{tab:DR_loss_results} where the run was for equal weights across classes.}\label{tab:DR_class_weighted}
%  \begin{center}
%\scalebox{0.7}{
%  \begin{tabular}{|r|r|r|r|r|r|r|r|r|}
%\toprule
%\multicolumn{5}{c}{\textbf{\underline{Class-adjusted weight}}} & \multicolumn{2}{c}{\textbf{\underline{Loss}}} & \multicolumn{2}{c}{\textbf{\underline{Accuracy}}}\\
%\textbf{Class 0} & \textbf{Class 1} & \textbf{Class 2} & \textbf{Class 3} & \textbf{Class 4} & \textbf{Training} & \textbf{Validation} & \textbf{Training} & \textbf{Validation}\\
%\midrule
%1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.6055 & 0.5985 & 0.7990 & 0.8106\\
%0.000004 & 0.00045 & 0.0002 & 0.0013 & 0.0016 & 1.0820 & 1.0840 & 0.6651 & 0.7390\\
%0.01 & 1 & 1 & 10 & 10 & 1.0917 & 1.0458 & 0.6494 & 0.6917\\
%0.25 & 1.0 & 0.85 & 1.0 & 1.0 & 0.8698 & 0.8662 & 0.7809 & 0.7926\\
%1 & 100 & 100 & 1000 & 10000 & 1.0913 & 1.0624 & 0.6624 & 0.7567\\
%\bottomrule
%\end{tabular}}
%\end{center}
%\end{table}
%
%\indent Lastly, the effect of using bilateral eye data was investigated. The rationale is that if either of a patient's eye meets criteria for referal from a screening, then the patient is referred for further evaluation. For example, if the right eye is Class 0, or normal, and the left eye is Class 3, or severe NPDR, then the patient is referred for further evaluation , then the patient is referred for further evaluation.\\
%\indent The Kaggle Diabetic Retinopathy data set consists of bilateral eye data. The test dataset consists of 53,576 images from 26,788 patients, where each patient contributed a right and left eye image. To analyze if performance could be increased, the test cases were ``blended'' from eye to patient level by assigning a diagnosis based on the eye with worse severity. This analysis was carried out for VGG-19 (pre-trained, fine-tuning), which showed accuracy of 73\%, sensitivity and specificity of 66\% and 90\% (for referable DR), and quadratic weighted kappa of 0.58. This was a decrease of 3.4\% in accuracy, an increase of 8.8\% in sensitivity, a decrease of 4.1\% in specificity, and an increase of 0.02 in quadratic weighted kappa compared to eye-level statistics.

